Learning from Contrastive Prompts: Automated Optimization and Adaptation

As LLMs evolve, significant effort is spent on manually crafting prompts. While existing prompt optimization methods automate this process, they rely solely on learning from incorrect samples, leading to a sub-optimal performance. Additionally, an unexplored challenge in the literature is prompts effective for prior models may not perform well on newer versions or different languages. We propose the Learning from Contrastive Prompts (LCP) framework to address these gaps, enhancing both prompt optimization and adaptation. LCP employs contrastive learning to generate effective prompts by analyzing patterns in good and bad prompt examples. Our evaluation on the Big-Bench Hard dataset shows that LCP has a win rate of over 76% over existing methods in prompt optimization and demonstrates strong adaptability across different model versions, families, and languages. LCP offers a systematic approach to prompt engineering, reducing manual effort in deploying LLMs across varied contexts.

==> old_tables/old_tables.tex <==
\begin{table}[t]
\small
\caption{Comparison of prompt optimization approaches: accuracy on BBH tasks for last iteration prompt (second for AutoHint) vs. best prompt. - indicates cases where AutoHint could not produce meaningful results.}
\label{table:op_perf}
\begin{center}
\begin{tabular}{lccc}
\hline
\multicolumn{1}{c}{\bf TASK}  &\multicolumn{1}{c}{\bf LCP} &\multicolumn{1}{c}{\bf AUTOHINT} &\multicolumn{1}{c}{\bf OPRO} \\
\hline
& \multicolumn{1}{c}{last / best of testing / best of training} & \multicolumn{1}{c}{last/best of testing} & \multicolumn{1}{c}{last/best of testing} \\
\hline
Algorithmic and Multi-Step Arithmetic Reasoning & & & \\
\hline
geometric\_shapes &  44.8 / \textbf{63.4} / 62.2 &  \textbf{45} / 45 & 33.5 / 33.5 \\
logical\_deduction\_three\_objects & \textbf{90.8} / \textbf{96.3} / 91.4  & 76 / 76  & 70.5 / 76 \\
logical\_deduction\_five\_objects & \textbf{70.5} / \textbf{76.9} / 68.0  & 52 / 52  & 54 / 65 \\
logical\_deduction\_seven\_objects & \textbf{62.8} / \textbf{67.8}  / 61.4 & 2 / 2  & 48 / 48.5 \\
penguins\_in\_a\_table & \textbf{97.2} / \textbf{98.5} \ 93.4 &  86.3 / 86.3 & 87.2 / 94.0 \\
reasoning\_about\_colored\_objects & 85.3 / 88.8 / 84.4 & 85.5 / 85.5  & \textbf{90.5} / \textbf{90.5} \\
temporal\_sequences &  \textbf{96.8} / \textbf{99.6} / 96.4 & - / - & 77.5 / 80 \\
tracking\_shuffled\_objects\_three\_objects & 96.8 / \textbf{99.5} / 98.7 & - / - & \textbf{99.5} / \textbf{99.5} \\
tracking\_shuffled\_objects\_five\_objects & \textbf{94.9} / \textbf{97.6} / 95.2 & - / - & 82.5 / 89.5 \\
tracking\_shuffled\_objects\_seven\_objects & \textbf{92.1} / \textbf{97.8} / 96.8 & - / - & 72.5 / 92 \\
\hline
Natural Language Understanding & & & \\
\hline
disambiguation\_qa & \textbf{67.0} / \textbf{72.8} / 60.3  &  55 / 57 & 50 / 50 \\
hyperbaton & \textbf{70.0} / \textbf{83.8} / 61.6  & 63 / 63  & 29 / 42.5 \\
salient\_translation\_error\_detection & 53.1 / \textbf{68.5} / 57.3 & \textbf{65} / 67  & 63 / 66.5 \\
snarks & 47.9 / 64.5 / 55.9 & \textbf{84.4} / \textbf{84.4} & 67.8 / 67.8 \\
\hline
Use of World Knowledge & & & \\
\hline
date\_understanding & 75.5 / \textbf{81.5} / 55.4  &  75.5 / 75.5 & \textbf{80.5} / 80.5 \\
movie\_recommendation & \textbf{75.9} / \textbf{83.6} \ 75.0 & 72 / 72  & 36 / 36 \\
ruin\_names & 65.9 / 78.0 / 63.9 & \textbf{76.5} / \textbf{79.5}  & 68 / 68 \\
\hline
Multilingual Knowledge and Reasoning & & & \\
\hline
salient\_translation\_error\_detection & 53.1 / \textbf{68.5} / 57.3 & \textbf{65} / 67  & 63 / 66.5 \\
\hline
Win Rates (\%) & \textbf{67.65} / \textbf{88.24} & 41.18 / 29.41 & 38.24 / 38.24 \\ \hline
\end{tabular}
\end{center}
\end{table}



\begin{table}[t]
\small
\caption{Comparison of prompt adaptation and prompt optimization on Claude-3-Sonnet: accuracy on BBH tasks for last iteration prompt vs. best prompt on the training set.}
\label{table:cross_version_perf}
\begin{center}
\begin{tabular}{lcc}
\hline
\multicolumn{1}{c}{\bf TASK}  &\multicolumn{1}{c}{\bf LCP Adaptation} &\multicolumn{1}{c}{\bf LCP Optimization} \\
\hline
& \multicolumn{1}{c}{last / best train / avg last 5} & \multicolumn{1}{c}{last /best train / avg last 5} \\
\hline
Algorithmic and Multi-Step Arithmetic Reasoning & & \\
\hline
geometric\_shapes & \textbf{70.5} / 65.5 / 67.8 & 44.8 / 62.2 / 69.0 \\
logical\_deduction\_three\_objects & \textbf{95.5} / 86.5 / 70.2 & 90.8 / 91.4 / 94.0\\
logical\_deduction\_five\_objects & 61.0 / 67.0 / 69.9 & \textbf{70.5} / 68.0 / 73.5 \\
logical\_deduction\_seven\_objects & 59.5 / 56.5 / 56.5 & \textbf{62.8} / 61.4 / 70.0 \\
penguins\_in\_a\_table & 93.2 / 93.2 / 92.3 & \textbf{97.2} / 93.4 / 94.9 \\
reasoning\_about\_colored\_objects & 82.5 / 85.0/ 84.5 & \textbf{85.3} / 84.4 / 86.0 \\
temporal\_sequences & 96.5 / 99.0 / 97.5 & \textbf{96.8} / 96.4 / 99.5 \\
tracking\_shuffled\_objects\_three\_objects & 91.0 / 92.5 / 93.6 & \textbf{96.8} / 98.7 / 99.0 \\
tracking\_shuffled\_objects\_five\_objects & 93.0 / 94.0 / 92.3 & \textbf{94.9} / 95.2 / 95.9 \\
tracking\_shuffled\_objects\_seven\_objects & \textbf{94.5} / 44.5 / 93.5 & 92.1 / 96.8 / 99.0 \\
\hline
Natural Language Understanding & & \\
\hline
disambiguation\_qa & 61.5 / 71.5 / 65.7 & \textbf{67.0} / 60.3 / 76.5 \\
hyperbaton & \textbf{82.0} / 83.0 / 79.2 & 70.0 / 61.6 / 82.5 \\
salient\_translation\_error\_detection &  \textbf{68.5} / 65.0 / 65.5 & 53.1 / 57.3 / 67.5 \\
snarks & \textbf{66.4} / 64.3 / 68.8 & 47.9 / 55.9 / 74.1 \\
\hline
Use of World Knowledge & & \\
\hline
date\_understanding & 73.5 / 73.5 / 74.2 & \textbf{75.5} / 55.4 / 76.0 \\
movie\_recommendation & 51.0 / 54.0 / 55.2 & \textbf{75.9} / 75.0 / 88.0 \\
ruin\_names & \textbf{76.5} / 80.0 / 77.7 & 65.9 / 63.9 / 78.0 \\
\hline
Multilingual Knowledge and Reasoning & & \\
\hline
salient\_translation\_error\_detection & \textbf{68.5} / 65.0 / 65.5 & 53.1 / 57.3 / 67.5 \\
\hline
Win Rates (\%) & 41.18 / 47.06 & \textbf{58.82} / \textbf{52.94} \\ \hline
\end{tabular}
\end{center}
\end{table}



\begin{table}[t]
\small
\caption{Comparison of prompt adaptation and prompt optimization on Claude-3-Haiku: accuracy on BBH tasks for last iteration prompt vs. best prompt.}
\label{table:cross_version_perf}
\begin{center}
\begin{tabular}{lcc}
\hline
\multicolumn{1}{c}{\bf TASK}  &\multicolumn{1}{c}{\bf LCP Adaptation} &\multicolumn{1}{c}{\bf LCP Optimization} \\
\hline
& \multicolumn{1}{c}{last / best train / avg last 5} & \multicolumn{1}{c}{last / best train / avg last 5} \\
\hline
Algorithmic and Multi-Step Arithmetic Reasoning & & \\
\hline
geometric\_shapes & \textbf{51.5} / 45.5 / \textbf{50.0} & 46.0 / 39.0 / 35.5\\
logical\_deduction\_three\_objects & \textbf{76.0} / 78.0 / \textbf{77.9} & 70.0 / 68.0 / 68.4 \\
logical\_deduction\_five\_objects & 50.0 / 56.0 / 49.0 & \textbf{55.0} / 50.0 / \textbf{52.8} \\
logical\_deduction\_seven\_objects & \textbf{42.5} / 47.0 / \textbf{45.1} & 7.0 / 46.0 / 22.0 \\
penguins\_in\_a\_table & \textbf{82.9} / 79.5 / \textbf{82.9} & 79.5 / 83.8 / 82.2 \\
reasoning\_about\_colored\_objects & 64.5 / 65.0 / \textbf{64.7} & \textbf{67.5} / 57.5 / 63.1 \\
temporal\_sequences & 83.5 / 89.5 / 88.4 & \textbf{93.0} / 93.8 / \textbf{94.1} \\
tracking\_shuffled\_objects\_three\_objects & 64.0 / 69.5 / 66.3 & \textbf{67.0} / 66.0 / \textbf{68.0}\\
tracking\_shuffled\_objects\_five\_objects & 43.0 / 60.0 / 46.7 & \textbf{67.5} / 68.0 / \textbf{64.5}\\
tracking\_shuffled\_objects\_seven\_objects & 55.0 / 56.5 / 58.2 & \textbf{62.5} / 61.5 / \textbf{61.7} \\
\hline
Natural Language Understanding & & \\
\hline
disambiguation\_qa & \textbf{67.0} / 69.5 / \textbf{65.7} & 61.0 / 62.0 / 62.9\\
hyperbaton & 87.0 / 90.0 / 86.8 & \textbf{88.0} / 84.0 / \textbf{89.9} \\
salient\_translation\_error\_detection & \textbf{56.5} / 58.0 / \textbf{54.8} & 51.5 / 52.0 / 51.8\\
snarks & \textbf{68.5} / 68.5 / \textbf{71.2} & 59.4 / 53.8 / 56.6\\
\hline
Use of World Knowledge & & \\
\hline
date\_understanding & \textbf{79.5} / 22.5 / \textbf{42.8} & 24.0 / 18.0 / 26.7\\
movie\_recommendation & 73.5 / 75.5 / \textbf{73.5} & \textbf{80.0} / 75.0 / 68.4\\
ruin\_names & 48.5 / 26.5 / 37.1 & \textbf{60.5} / 26.0 / \textbf{53.2} \\
\hline
Multilingual Knowledge and Reasoning & & \\
\hline
salient\_translation\_error\_detection & \textbf{56.5} / 58.0 / \textbf{54.8} & 51.5 / 52.0 / 51.8\\
\hline
Win Rates (\%) & 47.06 / \textbf{76.47} / \textbf{58.82} & \textbf{52.94} / 47.06 / 41.18\\ \hline
\end{tabular}
\end{center}
\end{table}





\begin{table}[t]
\small
\caption{Comparison of prompt adaptation and prompt optimization on Claude-3-Sonnet: accuracy on BBH tasks for last iteration prompt vs. best prompt on the training set.}
\label{table:cross_version_perf}
\begin{center}
\begin{tabular}{lcc}
\hline
\multicolumn{1}{c}{\bf TASK}  &\multicolumn{1}{c}{\bf LCP Adaptation} &\multicolumn{1}{c}{\bf LCP Optimization} \\
\hline
& \multicolumn{1}{c}{last / best train} & \multicolumn{1}{c}{last /best train} \\
\hline
Algorithmic and Multi-Step Arithmetic Reasoning & & \\
\hline
geometric\_shapes & \textbf{70.5} / \textbf{65.5} & 44.8 / 62.2 \\
logical\_deduction\_three\_objects & \textbf{95.5} / 86.5 & 90.8 / \textbf{91.4} \\
logical\_deduction\_five\_objects & 61.0 / 67.0 & \textbf{70.5} / \textbf{68.0} \\
logical\_deduction\_seven\_objects & 59.5 / 56.5 & \textbf{62.8} / \textbf{61.4} \\
penguins\_in\_a\_table & 93.2 / 93.2 & \textbf{97.2} / \textbf{93.4} \\
reasoning\_about\_colored\_objects & 82.5 / \textbf{85.0} & \textbf{85.3} / 84.4 \\
temporal\_sequences & 96.5 / \textbf{99.0} & \textbf{96.8} / 96.4 \\
tracking\_shuffled\_objects\_three\_objects & 91.0 / 92.5 & \textbf{96.8} / \textbf{98.7} \\
tracking\_shuffled\_objects\_five\_objects & 93.0 / 94.0 & \textbf{94.9} / \textbf{95.2} \\
tracking\_shuffled\_objects\_seven\_objects & \textbf{94.5} / 44.5 & 92.1 / \textbf{96.8} \\
\hline
Win Rates (\%) & 30.00 / 30.00 & 70.00 / 70.00 \\
\hline
Natural Language Understanding & & \\
\hline
disambiguation\_qa & 61.5 / \textbf{71.5} & \textbf{67.0} / 60.3 \\
hyperbaton & \textbf{82.0} / \textbf{83.0} & 70.0 / 61.6 \\
salient\_translation\_error\_detection &  \textbf{68.5} / \textbf{65.0} & 53.1 / 57.3 \\
snarks & \textbf{66.4} / \textbf{64.3} & 47.9 / 55.9 \\
\hline
Win Rates (\%) & 75.00 / 100.00 & 15.00 / 0.00 \\
\hline
Use of World Knowledge & & \\
\hline
date\_understanding & 73.5 / \textbf{73.5} & \textbf{75.5} / 55.4 \\
movie\_recommendation & 51.0 / 54.0 & \textbf{75.9} / \textbf{75.0} \\
ruin\_names & \textbf{76.5} / \textbf{80.0} & 65.9 / 63.9 \\
\hline
Win Rates (\%) & 33.33 / 66.67 & 66.67 / 33.33 \\
\hline
Multilingual Knowledge and Reasoning & & \\
\hline
salient\_translation\_error\_detection & \textbf{68.5} / \textbf{65.0} & 53.1 / 57.3 \\
\hline
Win Rates (\%) & 100.00 / 100.00 & 0.00 / 0.00 \\
\hline
Overall Win Rates (\%) & 41.18 / \textbf{52.94} & \textbf{58.82} / 47.06 \\ \hline
\end{tabular}
\end{center}
\end{table}

\begin{table}[t]
\small
\caption{Comparison of prompt adaptation and prompt optimization on Claude-3-Haiku: accuracy on BBH tasks for last iteration prompt vs. best prompt.}
\label{table:cross_version_perf}
\begin{center}
\begin{tabular}{lcc}
\hline
\multicolumn{1}{c}{\bf TASK}  &\multicolumn{1}{c}{\bf LCP Adaptation} &\multicolumn{1}{c}{\bf LCP Optimization} \\
\hline
& \multicolumn{1}{c}{last / best train } & \multicolumn{1}{c}{last / best train } \\
\hline
Algorithmic and Multi-Step Arithmetic Reasoning & & \\
\hline
geometric\_shapes & \textbf{51.5} / 45.5  & 46.0 / 39.0 \\
logical\_deduction\_three\_objects & \textbf{76.0} / 78.0 & 70.0 / 68.0 \\
logical\_deduction\_five\_objects & 50.0 / 56.0 & \textbf{55.0} / 50.0 \\
logical\_deduction\_seven\_objects & \textbf{42.5} / 47.0 & 7.0 / 46.0 \\
penguins\_in\_a\_table & \textbf{82.9} / 79.5 & 79.5 / 83.8 \\
reasoning\_about\_colored\_objects & 64.5 / 65.0 & \textbf{67.5} / 57.5 \\
temporal\_sequences & 83.5 / 89.5 & \textbf{93.0} / 93.8 \\
tracking\_shuffled\_objects\_three\_objects & 64.0 / 69.5 & \textbf{67.0} / 66.0 \\
tracking\_shuffled\_objects\_five\_objects & 43.0 / 60.0 & \textbf{67.5} / 68.0 \\
tracking\_shuffled\_objects\_seven\_objects & 55.0 / 56.5 & \textbf{62.5} / 61.5 \\
\hline
Win Rates (\%) &  & \\ 
\hline
Natural Language Understanding & & \\
\hline
disambiguation\_qa & \textbf{67.0} / 69.5 & 61.0 / 62.0 \\
hyperbaton & 87.0 / 90.0 & \textbf{88.0} / 84.0 \\
salient\_translation\_error\_detection & \textbf{56.5} / 58.0 & 51.5 / 52.0 \\
snarks & \textbf{68.5} / 68.5 & 59.4 / 53.8 \\
\hline
Win Rates (\%) &  & \\ 
\hline
Use of World Knowledge & & \\
\hline
date\_understanding & \textbf{79.5} / 22.5 & 24.0 / 18.0 \\
movie\_recommendation & 73.5 / 75.5 & \textbf{80.0} / 75.0 \\
ruin\_names & 48.5 / 26.5 & \textbf{60.5} / 26.0 \\
\hline
Win Rates (\%) &  & \\ 
\hline
Multilingual Knowledge and Reasoning & & \\
\hline
salient\_translation\_error\_detection & \textbf{56.5} / 58.0 & 51.5 / 52.0 \\
\hline
Win Rates (\%) &  & \\ 
\hline
Overall Win Rates (\%) &  & \\ 
\hline
\end{tabular}
\end{center}
\end{table}
